AR2-D2:Training a Robot Without a Robot

Diligently gathered human demonstrations serve as the unsung heroes empowering the progression of robot learning. Today, demonstrations are collected by training people to use specialized controllers, which (tele-)operate robots to manipulate a small number of objects. By contrast, we introduce AR2-D2: a system for collecting demonstrations which (1) does not require people with specialized training, (2) does not require any real robots during data collection, and therefore, (3) enables manipulation of diverse objects with a real robot. AR2-D2 is a framework in the form of an iOS app that people can use to record a video of themselves manipulating any object while simultaneously capturing essential data modalities for training a real robot. We show that data collected via our system enables the training of behavior cloning agents in manipulating real objects. Our experiments further show that training with our AR data is as effective as training with real-world robot demonstrations. Moreover, our user study indicates that users find AR2-D2 intuitive to use and require no training in contrast to four other frequently employed methods for collecting robot demonstrations.

==> old/abstract_v1.tex <==
% In recent years, the field of robotics has seen remarkable advancements, resulting in the development of more complex and sophisticated robots. Training these robots using reinforcement learning can be time-consuming and challenging. Imitation learning, where robots learn by observing and copying expert demonstrations, has emerged as a promising solution. However, the quality of expert demonstrations plays a critical role in determining the success of the imitation learning process. In this paper, we propose an innovative method for collecting robotic demonstrations called JARVIS (Just Use Augmented Reality for Collecting Multi-Task Demonstrations in Personalized Environments). JARVIS is an augmented reality iOS mobile application that enables users to project a fully functional robot into their real-world environment and collect demonstrations using various control mechanisms. We compare the performance of models trained using different forms of data (Real, Simulation, AR) on a shared task and experimental setting. Our results indicate that there exists a large domain gap between various settings, which data is collected from, highlighting the importance of choosing suitable tasks and data collection approaches for effective robotic learning.

==> old/abstract_v2.tex <==


Painstakingly-collected human demonstrations are the inglorious heroes enabling robot learning.
Today, demonstrations are collected by training people to use specialized controllers, which (tele-)operate robots to manipulate a small number of objects.
By contrast, we introduce \system: a system for collecting demonstrations (1) without the need to train people, (2) without any real robots, and therefore, (3) enabling manipulation of diverse objects.
\system\ is an iOS app that people can use to record a video of themselves manipulating any object. Once the video is captured, \system\ uses the iOS depth sensor to place an AR robot in the scene and uses inverse kinetics to produce a trajectory where it appears as if the AR robot manipulates the object.
We show that with as few as five effortless AR demonstrations, we can train a real robot to manipulate real objects.
Our experiments show that training with \system's AR data is as effective as training with real-world demonstrations.
Moreover, our user study indicates that users find \system\ intuitive to use and require no training when compared to five other collection methods; users also produce demosntrations as fast as kinesthetic-teaching.


==> old/experiments_v1.tex <==
\section{Evaluating \system\ with a real robot deployment}

% MAIN RESULTS:
% 2: robot can learn to manipulate objects that have never been interacted with a real robot. 
% 3: can now train a robot to interact with a personalized objects that is not obtainable en masse
% 4: manipulation results are as successful as those collected using real demonostrations with a real robot
% minor ablations: optimal number of demonstrations for finetuning, rbg-only variants, learning from simulation.

\begin{table*}[t]
\begin{center}
    \resizebox{\textwidth}{!}{%z
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|}
    \hline
     {Methods/Skills}&  \multicolumn{3}{|c|}{Press (\emph{Succ.\%})}& \multicolumn{3}{|c|}{Push (\emph{Succ.\%})}& \multicolumn{3}{|c|}{Pick (\emph{Succ.\%})}\\
    \hline
    Personalized Object& Computer Mouse & Minecraft Torch & Cross Button & LEGO Train & 8 Ball  & Drawer & Chess Piece & Bowl & Paper Bag \\
    \hline
    Simulation &  13.3 & 6.7&30.0 &13.3 &20.0 &3.3&3.3&20.0 &16.7 \\
    \hline
    PerAct VR interface (w/o personalized objects)& 3.3 & 6.7& 16.7& 13.3 & 10.0 & 3.3& 0.0& 10.0&6.7 \\
    \hline
    PerAct VR interface (with personalized objects)& \textbf{60.0} & \textbf{63.3} & \textbf{83.3} & 30.0 & \textbf{70.0} & \textbf{40.0} & \textbf{46.7} & \textbf{56.7} & 60.0\\
    \hline
       AR2-D2 (Ours) &56.7 & 53.3 & 73.3 & \textbf{50.0} &55.7 &23.3 &\textbf{46.7} &53.3 & \textbf{63.3} \\
    \hline

    


    \end{tabular}
    }
\end{center}
\caption{\textbf{Task Test Results}. Success rates (mean \%) of the foundational skills being tested on the personalized objects collected via AR2-D2. For each foundational skills, we evaluate it across ten different sets of distractors with the target object and repeated each three times for consistency. The result has shown that our approach of data collection with minimal fine-tuning obtains comparable results to real-world data collected on these personalized objects via PerAct's VR interface with a physical robot.}
\label{tab:press_push_pick_table}
\end{table*}



\subsection{Training Strategy}

We develop our training strategy based on the core purpose of   AR2-D2, that is, to enable collection of demonstrations with personalized objects in custom environments. Hence, we collect demonstrations using   AR2-D2 on a series of personalized objects, and demonstrate the policy execution on a real Franka-Emika Panda robot for skills involving the personalized objects.

To train using the demonstrations collected via   AR2-D2, we employ Perciver-Actor (PerAct) \cite{shridhar2022perceiver}, a transformer-based language-guided behavior cloning policy. PerAct takes a 3D voxel observation and a language goal $(v, l)$ as input and produces discretized outputs for translation, rotation, and gripper state of the end-effector. These outputs, coupled with a motion planner, enables execution of the task specified by the language goal.

Data collection for training is done using   AR2-D2, and the VR interface from PerAct \cite{shridhar2022perceiver}. The VR interface from PerAct involves using a VR handset to guide the real-robot to desired end-effector poses. We gather demonstrations centered around three foundational skills: $S=$ \{\emph{press, push, pick}\}. Using the VR system from PerAct, we collect 5 sets of demonstrations using three dummy objects: $O=$ \{\emph{red button, yellow block, tennis ball}\}, corresponding to the three foundational skills, respectively. For   AR2-D2, we also collect five sets of demonstrations using three distinctively different objects, which vary in colour, geometry, and texture.

Following the procedure from PerAct, we train an individual model for each foundational skill. To train the model for a given skill, we undergo a training phase consisting of 30,000 iterations per set of demonstrations. We then freeze the backbone of the PerAct architecture and finetune using the set of VR collected demonstrations on those dummy objects corresponding to the given skill. This fine-tuning process spans an additional 3,000 iterations, equivalent to approximately 10 minutes. The need for fine-tuning arises due to the domain gap resulting from differences in depth cameras between the Kinect V2 and the Stereo depth camera on the iPad, from which   AR2-D2 collects data.

During testing, we exclusively evaluate the pre-trained   AR2-D2-PerAct model on the distinctly different objects from the   AR2-D2-enabled real-world demonstrations. To ensure consistency, we evaluate across ten different sets of distractors, and repeat three times for each setting to obtain the average performance. The rationale behind this training strategy is to demonstrate that with   AR2-D2, we can collect personalized objects in custom environments, enabling training and facilitating the model's ability to generalize and manipulate these objects. The fine-tuning stage serves as a grounding process, allowing the model to adapt to the existing environment. We also evaluated directly using   AR2-D2 demonstrations which was trained on PerAct for 30,000 iterations and with no fine-tuning in our ablation study.

% To train using the demonstrations collected via   AR2-D2, we employ Perciver-Actor (PerAct) \cite{shridhar2022perceiver}, a transformer-based language-guided behavior cloning policy. PerAct takes a 3D voxel observation and a language goal $(v, l)$ as input and produces discretized outputs for translation, rotation, and gripper state of the end-effector. These outputs, coupled with a motion planner, enables execution of the task specified by the language goal.

% To ensure   AR2-D2 demonstrations are effective in real-world scenarios with PerAct, a small amount of fine-tuning is required. This fine-tuning process involves utilizing a few real-world demonstrations collected via PerAct. The need for fine-tuning arises due to the domain gap resulting from differences in depth cameras between the Kinect V2 and the Stereo depth camera on the iPad, from which the data was collected. The fine-tuning duration is less than $\approx 10 minutes$.

% To evaluate the quality and usefulness of the collected   AR2-D2 demonstrations, we initially gather 3 sets of 5 demonstrations for three foundational skills: $S=$ \{\emph{press, push, pick}\} on three simple objects:$O=$ \{\emph{red button, yellow block, tennis ball}\}. These demonstrations are obtained using PerAct's VR interface. Subsequently, based on these foundational skills, we collect 5 demonstrations each on three different objects at personalized environment, varying in terms of colors, geometric shapes, and textures using   AR2-D2. This evaluation process allows us to assess the quality of   AR2-D2-collected demonstrations.

% For each new set of demonstrations, collected on individual skills, we undergo a training phase consisting of 30,000 iterations. Afterward, we freeze the backbone of the PerAct architecture and proceed to fine-tune it using the initial demonstrations specific to the corresponding foundational skill, which were collected via PerAct's VR interface. This fine-tuning process spans an additional 3,000 iterations, equivalent to approximately 10 minutes. During testing, we exclusively evaluate the pre-trained   AR2-D2-PerAct model on the distinctly different objects from the real-world demonstrations and across ten different sets of distractor for three times to obtain the average performance.. The rationale behind this training strategy is to demonstrate that with   AR2-D2, we can collect personalized objects in custom environments, enabling training and facilitating the model's ability to generalize and manipulate these objects. The fine-tuning stage serves as a grounding process, allowing the model to adapt to the existing environment.


\subsection{Baseline Collection Methods}

To evaluate the effectiveness of our approach, we compared it with two alternative methods of demonstration collection: real-world and simulation data collection. However, we fine-tuned all three methods using the same set of demonstrations collected from the real world, and subsequently evaluated their performance in identical real-world conditions.

\textbf{Real World.} For the real-world data collection method, we utilized the VR controller interface to capture the training demonstrations, as described in PerAct \cite{shridhar2022perceiver}. For the real-world demonstrations collections, we further benchmark our approach with real-world data collected for the personalized objects and without the personalized objects being used for the demonstration skills, which is known as PerAct (w/o the personalized objects) and PerAct(with the personalized objects) as shown in Table 1.

\textbf{Simulation.} For the simulation demonstrations, we employed RLBench and its key-frame point extraction technique to acquire the data, accompanied by motion planning to generate each demonstration within the simulation environment. Furthermore, in the case of simulation demonstrations, we implemented domain randomization for the purpose of introducing texture variations, aiding in the transfer of skills from simulation to the real world.



\subsection{Training Details} 
For training PerAct \cite{shridhar2022perceiver}, the voxel grid size employed was $100^3$, while the image resolution used was [512, 424]. The training of the agents was performed using three NVIDIA 3090 RTX GPUs. For training, we introduce $\pm0.125 m$ translation perturbations and $\pm 45 ^\circ$ yaw rotation perturbations. The LAMB \cite{lamb} optimizer was used following Perceiver \cite{perceivertransformer}.

% We conducted training experiments involving the baseline methods of demonstration collection through the utilization of PerAct. The voxel grid size employed was $100^3$, while the image resolution used was [512, 424]. The training of the agents was performed using three NVIDIA 3090 RTX GPUs. To evaluate the effectiveness of our approach, we compared it with two alternative methods of demonstration collection: real-world and simulation data collection. However, we fine-tuned all three methods using the same set of demonstrations collected from the real world, and subsequently evaluated their performance in identical real-world conditions.



\subsection{Results and Ablative Studies}
\begin{wrapfigure}{r}{0.4\textwidth}
%   \vspace{-1.3em}
%   \vspace{-2.3em}
%   \vspace{-4.3em}
  
  \begin{center}
    \vspace{-0.8cm}
    % \hspace{2.5cm}
    \includegraphics[width=0.42\textwidth]{images/diagnostic (2).png}

%   \vspace{-1.2em}
  \vspace{-0.05cm}
  \caption{\textbf{Analysis on Fine-tuning.} We have further undertaken a diagnostic analysis to determine the minimum necessary number of iterations and demonstrations required to achieve optimal performance. This analysis involved varying the number of demonstrations and iterations for fine-tuning.}
  \label{fig:ablations}
  \end{center}
  \vspace{-2em}
%   \vspace{-1.7em}
%   \vspace{-0.5em}
\end{wrapfigure}
\vspace{-0.05cm}
\textbf{Real-world Result.} 
Table \ref{tab:press_push_pick_table} reports success rates of all the nine personalized objects during test time with the demonstration data collected via the baseline collection methods.  In order to ensure fairness and consistency in evaluating the various methods, we conducted tests on the trained models using ten different sets of distractors. Additionally, we repeated the tests three times with different table top configurations to obtain the average performance.

In general the demonstration data collected either through simulation or using the PerAct VR interface (without the inclusion of personalized objects) tends to underperform due to the unavailability of these personalized objects, which are presented during testing. These findings underscore the significance of our approach, which facilitates access to collecting demonstrations with such personalized objects. Moreover, they indicate that behavior cloning (BC) models, such as PerAct, require exposure to analogous objects during demonstration to successfully execute tasks involving these objects during testing. More importantly, referencing Table \ref{tab:press_push_pick_table}, it is evident that even with the integration of these personalized objects during the demonstration data collection phase, our methods deliver comparable results to data amassed via PerAct's VR interface using a real robot. Remarkably, our system even surpasses the performance of the PerAct VR Interface (which incorporates personalized objects) in tasks such as pushing the LEGO train and picking up the paper bag. While for the remaining personalized objects, our approach maintaining a $\leq 14.3 \% $ across the three foundational skills.


% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=\linewidth]{images/diagnostic (2).png}
%     \caption{Your Figure}
%     \label{fig:fig5}
% \end{figure}




% \begin{wrapfigure}{r}{0.4\textwidth}
% %   \vspace{-1.3em}
% %   \vspace{-2.3em}
% %   \vspace{-4.3em}
  
%   \begin{center}
%     \vspace{-0.8cm}
%     % \hspace{2.5cm}
%     \includegraphics[width=0.42\textwidth]{diagnostic.png}

% %   \vspace{-1.2em}
%   \vspace{-0.05cm}
%   \caption{\textbf{Ablation Experiments.} Success rate of \model~after ablating key components.}
%   \label{fig:your_figure}
%   \end{center}
%   \vspace{-1em}
% %   \vspace{-1.7em}
% %   \vspace{-0.5em}
% \end{wrapfigure}
% \vspace{-0.4em}
% \hspace{-2.5cm}
% \vspace{-0.05cm}
% \textbf{Ablations.} \tabref{table:rlbench} reports \model~w/o Lang, an agent without any language conditioning. Without a language goal, the agent does not know the underlying task and performs at chance. We also report additional ablation results on the \texttt{open drawer} task in \figref{fig:ablations}. To summarize these results: (1) the skip connection helps train the agent slightly faster, (2) the Perceiver Transformer is crucial for achieving good performance with the global receptive field, and (3) extracting good keyframes actions is essential for supervised training as randomly chosen or fixed-interval keyframes lead to zero-performance.
\begin{wraptable}{r}{0.52\textwidth}
  %\begin{table}[h]
%   \hspace*{-1em}
%   \vspace{-0.5cm}
  \vspace{-1.3em}
  \setlength\tabcolsep{2.3pt}
  \centering
  \scriptsize
\begin{tabular}{lcc} 
\toprule
Task          & 2D data (Image-BC)~ & 3D data (PerAct)  \\ 
\midrule
Press the buzzer from the side & 6.67\%         & 40.00\%    \\
Pick up the queen piece    & 6.67\%         & 33.34\%           \\
Press the computer mouse    & 40.00\%        & 40.00\%           \\
\bottomrule
\end{tabular}
%   \vspace{-0.5em}
    \caption{\textbf{Training with Different Data Modalities.} AR2-D2 is capable of offering diverse data modalities to facilitate training BC models, such as Image-BC for 2D data and PerAct for 3D data. We assess these disparate data modalities, gathered via AR2-D2, across three distinct tasks using Image-BC for 2D data and PerAct for 3D data, conducted without any form of fine-tuning} % task, success \% vs. $\#$ of demonstrations. 
  \vspace{-2em}
  \label{table:table2}
\end{wraptable}
\textbf{Analysis on Fine-tuning.} To find the most effective iteration and demonstration combination for real-world fine-tuning, we conduct an analysis by varying the number of fine-tuning demonstrations, $D = \{1, 3, 5, 10, 15\}$, and iterations, $I = \{0, 1000, 2000, 3000, 4000, 5000\}$, during model fine-tuning and measuring the corresponding success rate. Specifically, for pre-training, we use five demonstrations totalling 30,000 iterations of the ``mouse" pressing task, collected using   AR2-D2. Following pre-training, we fine-tune with real-world demonstrations. Each resulting model is tested on five real-world scenes which has varying target object poses and distraction objects. We illustrate the experimental results in Table \ref{fig:ablations}, which indicate that utilizing 5 demonstrations of real-world foundational skills and training for 3,000 iterations (equivalent to 10 minutes of training) yields the most effective outcome.

% In Figure \ref{fig:diagnostic_analysis}, we investigate the relationship between the number of real-world fine-tuning demonstrations and the number of iterations for fine-tuning  towards the performances of tasks for demonstrations collected via   AR2-D2.  We conducted an analysis by gathering five demonstrations of pressing the "mouse" using   AR2-D2 and pre-training it for 30,000 iterations. Subsequently, we fine-tuned the pre-trained model by varying the number of real-world demonstrations and training iterations in five different instances of a test scene, with the positions of the target object and distractor also varied. This allowed us to calculate the average success rate for each combination of demonstrations and iterations. The results of this diagnostic study indicate that utilizing 5 demonstrations of real-world foundational skills and training for 3,000 iterations (equivalent to 10 minutes of training) yielded the most effective outcomes.


\textbf{Training with Different Data Modalities.} \system facilitates collection of both 2D image data and 3D depth data, which enables training of both image-based behaviour cloning (Image-BC) and 3D voxelized methods like PerAct \cite{shridhar2022perceiver}. In Table \ref{table:table2}, we show the performance of Image-BC and PerAct, trained using 2D image and 3D voxel input, respectively. We demonstrate that in a zero-shot setting, where the training data is collected in AR using \system and inference is run directly on real-world sensor input without fine-tuning, \system enables successful task execution for pushing, picking, and pressing style tasks. Specifically, we find that while models trained using 2D and 3D are capable of performing pushing, picking, and pressing style tasks, incorporating 3D information enhances the success rate by a large margin, as shown in Figure Table \ref{table:table2}. 

% of  data  enable some level of successful task execution. However, when 3D information is incorporated, the success rate significantly outperforms the Image-BC which only incorporates 2D information. 


% image data only, the Image-BC model achieves Specifically,   leverages real-world data is directly run on the for the task of \emph{pressing the cross button from the side}, in a zero-shot setting (without finetuning), we can achieve...

% To investigate the validity of different modalities collected using \system, we leverage the data to train an image-based behaviour cloning agent and Perceiver Actor. 


% To demonstrate the  To investigate the  

% Figure XXX presents an experiment investigating the influence of various input data modalities on the performance of behavior cloning agents trained to execute the task of \emph{pressing the cross button from the side}, which necessitates rotating the robot's end-effector. The experiment involves two models, namely PerAct \cite{shridhar2022perceiver} and Image-BC, and three sets of input modalities. 


% 1) train a image-BC agent, which is an image-to-action
% agent similar to BC-Z [12]. The image-BC model using RGB frames generated through our cross-reality perception pipeline. 2) A 3D voxel inputs from the    AR2-D2 onboard device sensor, which are combined with real-world action demonstrations and fine-tuned on the PerAct model. 3) A 3D voxel inputs from the    AR2-D2 onboard device sensor without any fine-tuning. All of these three models are trained for 30,000 iterations on 5 demonstrations collected via    AR2-D2.

% Figure XXX presents an experiment investigating the influence of various input data modalities on the performance of behavior cloning agents trained to execute the task of \emph{pressing the cross button from the side}, which necessitates rotating the robot's end-effector. The experiment involves two models, namely PerAct and Image-BC, and three sets of input modalities. 1) training the Image-BC model using RGB frames generated through our cross-reality perception pipeline. 2) A 3D voxel inputs from the    AR2-D2 onboard device sensor, which are combined with real-world action demonstrations and fine-tuned on the PerAct model. 3) A 3D voxel inputs from the    AR2-D2 onboard device sensor without any fine-tuning. All of these three models are trained for 30,000 iterations on 5 demonstrations collected via    AR2-D2.



==> old/experiments_v2.tex <==
\section{Evaluating \system\ with a real robot deployment}

% \rk{Ok, I would like you to edit this section by yourself. Look at the other sections to make sure you say things in the same consistent way. The most important thing to do first is to set up expectations for the reader. What exactly is the main take away message from this section. Read Cheng-Yu's Distill or Zixian's CREPE papers to see how experiments sections are laid out. Here is the general guideline I recommend:

% 1. Your first paragraph should cover the main takeaways from the results. One sentence per takeaway.

% 2. You need paragraphs for experimental setup: how is training done? What are the metrics? How is the data collected between different methods?

% 3. Next you need a subsection or paragraph per main takeaway. The first sentence of each paragraph should be bolded with the takeaway. The rest of the sentences should lay out the details.
% }

We present our results and experiments and highlight two main takeaways. First, we show that using \system, we can collect demonstrations with personalized objects without access to a physical robot, and train manipulation policies that can interact with the personalized objects in the real world. Second, we demonstrate that the manipulation results across different tasks trained with \system demonstrations are on-par with those collected using real robot demonstrations. Third, we show experiments which use data collected using \system with a variety of training schemes, and show that \system enables training with varied finetuning iterations and input modality.

% MAIN RESULTS:
% 2: robot can learn to manipulate objects that have never been interacted with a real robot. 
% 3: can now train a robot to interact with a personalized objects that is not obtainable en masse
% 4: manipulation results are as successful as those collected using real demonostrations with a real robot
% minor ablations: optimal number of demonstrations for finetuning, rbg-only variants, learning from simulation.

\begin{table*}[t]
\begin{center}
    \resizebox{\textwidth}{!}{%z
    \begin{tabular}{l p{0.2pt}ccc p{0.2pt}ccc p{0.2pt}ccc}
    \toprule
     Task& & \multicolumn{3}{c}{Press (\emph{Succ.\%})}&& \multicolumn{3}{c}{Push (\emph{Succ.\%})}&& \multicolumn{3}{c}{Pick up (\emph{Succ.\%})}\\
    \cline{3-5}\cline{7-9}\cline{11-13}
    Personalized object&& Computer mouse & Minecraft torch & Buzzer && LEGO train & 8 ball  & Drawer && Queen piece & Plastic bowl & Takeaway bag \\
    \midrule
    Simulation &&  13.3 & 6.7&30.0 &&13.3 &20.0 &3.3&&3.3&20.0 &16.7 \\
    PerAct VR interface (w/o personalized objects)&& 3.3 & 6.7& 16.7&& 13.3 & 10.0 & 3.3&& 0.0& 10.0&6.7 \\
    PerAct VR interface (with personalized objects)&& \textbf{60.0} & \textbf{63.3} & \textbf{83.3} && 30.0 & \textbf{70.0} & \textbf{40.0} && \textbf{46.7} & \textbf{56.7} & 60.0\\
       AR2-D2 (Ours) &&56.7 & 53.3 & 73.3 && \textbf{50.0} &55.7 &23.3 &&\textbf{46.7} &53.3 & \textbf{63.3}\\
    \bottomrule
    
    \end{tabular}
    }
\end{center}
\caption{\textbf{Task Test Results}. Success rates (mean \%) of the foundational skills being tested on the personalized objects collected via AR2-D2. For each foundational skills, we evaluate it across ten different sets of distractors with the target object and repeated each three times for consistency. The result has shown that our approach of data collection with minimal fine-tuning obtains comparable results to real-world data collected on these personalized objects via PerAct's VR interface with a physical robot.}
\label{tab:press_push_pick_table}
\end{table*}



\subsection{Experimental Setup}



We develop our training strategy based on the core purpose of   AR2-D2, that is, to enable collection of demonstrations with personalized objects in custom environments. Hence, we collect demonstrations using   AR2-D2 on a series of personalized objects, and demonstrate the policy execution on a real Franka-Emika Panda robot for skills involving the personalized objects.

\textbf{Behaviour Cloning Architecture.} To train using the demonstrations collected via   AR2-D2, we employ Perciver-Actor (PerAct) \cite{shridhar2022perceiver}, a transformer-based language-guided behavior cloning policy. PerAct takes a 3D voxel observation and a language goal $(v, l)$ as input and produces discretized outputs for translation, rotation, and gripper state of the end-effector. These outputs, coupled with a motion planner, enables execution of the task specified by the language goal.

\textbf{Demonstration Collection.} Data collection for training is done using \system, and the VR interface from PerAct \cite{shridhar2022perceiver}. The VR interface from PerAct involves using a VR handset to guide the real-robot to desired end-effector poses. We gather demonstrations centered around three foundational skills: $S=$ \{\emph{press, push, pick up}\}. Using the VR system from PerAct, we collect 5 sets of demonstrations using three dummy objects: $O=$ \{\emph{red button, yellow block, tennis ball}\}, corresponding to the three foundational skills, respectively. For   AR2-D2, we also collect five sets of demonstrations using three distinctively different objects, which vary in colour, geometry, and texture.

\textbf{Training Procedure.} Following the procedure from PerAct, we train an individual model for each foundational skill. To train the model for a given skill, we undergo a training phase consisting of 30,000 iterations per set of demonstrations. We then freeze the backbone of the PerAct architecture and finetune using the set of VR collected demonstrations on those dummy objects corresponding to the given skill. This fine-tuning process spans an additional 3,000 iterations, equivalent to approximately 10 minutes. The need for fine-tuning arises due to the domain gap resulting from differences in depth cameras between the Kinect V2 and the Stereo depth camera on the iPad, from which   AR2-D2 collects data.

\textbf{Testing Procedure.} During testing, we exclusively evaluate the pre-trained   AR2-D2-PerAct model on the distinctly different objects from the   AR2-D2-enabled real-world demonstrations. To ensure consistency, we evaluate across ten different sets of distractors, and repeat three times for each setting to obtain the average performance. The rationale behind this training strategy is to demonstrate that with   AR2-D2, we can collect personalized objects in custom environments, enabling training and facilitating the model's ability to generalize and manipulate these objects. The fine-tuning stage serves as a grounding process, allowing the model to adapt to the existing environment. We also evaluated directly using   AR2-D2 demonstrations which was trained on PerAct for 30,000 iterations and with no fine-tuning in our ablation study.

\textbf{Baselines.} To evaluate the effectiveness of our approach, we compared it with two alternative methods of demonstration collection: real-world and simulation data collection. However, we fine-tuned all three methods using the same set of demonstrations collected from the real world, and subsequently evaluated their performance in identical real-world conditions. \textit{Real world} data collection involves a VR controller interface to capture the training demonstrations, as described in PerAct \cite{shridhar2022perceiver}. For the real-world demonstrations collections, we benchmark our approach with real-world demonstrations collected with and without the personalized objects, denoted as PerAct (w/o personalized objects) and PerAct (with personalized objects), respectively, as shown in Table \ref{tab:press_push_pick_table}. \textit{Simulation} demonstrations involves RLBench and its key-frame point extraction technique, accompanied by motion planning to generate each demonstration within the simulation environment \cite{rlbench}. Furthermore, in the case of simulation demonstrations, we implemented domain randomization for the purpose of introducing texture variations, aiding in the transfer of skills from simulation to the real world.

% To train using the demonstrations collected via   AR2-D2, we employ Perciver-Actor (PerAct) \cite{shridhar2022perceiver}, a transformer-based language-guided behavior cloning policy. PerAct takes a 3D voxel observation and a language goal $(v, l)$ as input and produces discretized outputs for translation, rotation, and gripper state of the end-effector. These outputs, coupled with a motion planner, enables execution of the task specified by the language goal.

% To ensure   AR2-D2 demonstrations are effective in real-world scenarios with PerAct, a small amount of fine-tuning is required. This fine-tuning process involves utilizing a few real-world demonstrations collected via PerAct. The need for fine-tuning arises due to the domain gap resulting from differences in depth cameras between the Kinect V2 and the Stereo depth camera on the iPad, from which the data was collected. The fine-tuning duration is less than $\approx 10 minutes$.

% To evaluate the quality and usefulness of the collected   AR2-D2 demonstrations, we initially gather 3 sets of 5 demonstrations for three foundational skills: $S=$ \{\emph{press, push, pick}\} on three simple objects:$O=$ \{\emph{red button, yellow block, tennis ball}\}. These demonstrations are obtained using PerAct's VR interface. Subsequently, based on these foundational skills, we collect 5 demonstrations each on three different objects at personalized environment, varying in terms of colors, geometric shapes, and textures using   AR2-D2. This evaluation process allows us to assess the quality of   AR2-D2-collected demonstrations.

% For each new set of demonstrations, collected on individual skills, we undergo a training phase consisting of 30,000 iterations. Afterward, we freeze the backbone of the PerAct architecture and proceed to fine-tune it using the initial demonstrations specific to the corresponding foundational skill, which were collected via PerAct's VR interface. This fine-tuning process spans an additional 3,000 iterations, equivalent to approximately 10 minutes. During testing, we exclusively evaluate the pre-trained   AR2-D2-PerAct model on the distinctly different objects from the real-world demonstrations and across ten different sets of distractor for three times to obtain the average performance.. The rationale behind this training strategy is to demonstrate that with   AR2-D2, we can collect personalized objects in custom environments, enabling training and facilitating the model's ability to generalize and manipulate these objects. The fine-tuning stage serves as a grounding process, allowing the model to adapt to the existing environment.


% \subsection{Baseline Collection Methods}

% To evaluate the effectiveness of our approach, we compared it with two alternative methods of demonstration collection: real-world and simulation data collection. However, we fine-tuned all three methods using the same set of demonstrations collected from the real world, and subsequently evaluated their performance in identical real-world conditions.

% \textbf{Real World.} For the real-world data collection method, we utilized the VR controller interface to capture the training demonstrations, as described in PerAct \cite{shridhar2022perceiver}. For the real-world demonstrations collections, we further benchmark our approach with real-world data collected for the personalized objects and without the personalized objects being used for the demonstration skills, which is known as PerAct (w/o the personalized objects) and PerAct (with the personalized objects), respectively, as shown in Table \ref{tab:press_push_pick_table}.

% \textbf{Simulation.} For the simulation demonstrations, we employed RLBench and its key-frame point extraction technique to acquire the data, accompanied by motion planning to generate each demonstration within the simulation environment. Furthermore, in the case of simulation demonstrations, we implemented domain randomization for the purpose of introducing texture variations, aiding in the transfer of skills from simulation to the real world.



% \subsection{Training Details} 
% For training PerAct \cite{shridhar2022perceiver}, the voxel grid size employed was $100^3$, while the image resolution used was [512, 424]. The training of the agents was performed using three NVIDIA 3090 RTX GPUs. For training, we introduce $\pm0.125 m$ translation perturbations and $\pm 45 ^\circ$ yaw rotation perturbations. The LAMB \cite{lamb} optimizer was used following Perceiver \cite{perceivertransformer}.

% We conducted training experiments involving the baseline methods of demonstration collection through the utilization of PerAct. The voxel grid size employed was $100^3$, while the image resolution used was [512, 424]. The training of the agents was performed using three NVIDIA 3090 RTX GPUs. To evaluate the effectiveness of our approach, we compared it with two alternative methods of demonstration collection: real-world and simulation data collection. However, we fine-tuned all three methods using the same set of demonstrations collected from the real world, and subsequently evaluated their performance in identical real-world conditions.



\subsection{Results}
\begin{wrapfigure}{r}{0.4\textwidth}
%   \vspace{-1.3em}
%   \vspace{-2.3em}
%   \vspace{-4.3em}
  
  \begin{center}
    \vspace{-0.8cm}
    % \hspace{2.5cm}
    \includegraphics[width=0.42\textwidth]{images/diagnostic (2).png}

%   \vspace{-1.2em}
  \vspace{-0.05cm}
  \caption{\textbf{Analysis on Fine-tuning.} We have further undertaken a diagnostic analysis to determine the minimum necessary number of iterations and demonstrations required to achieve optimal performance. This analysis involved varying the number of demonstrations and iterations for fine-tuning.}
  \label{fig:ablations}
  \end{center}
  \vspace{-2em}
%   \vspace{-1.7em}
%   \vspace{-0.5em}
\end{wrapfigure}
\vspace{-0.05cm}

Table \ref{tab:press_push_pick_table} reports success rates of all the nine personalized objects during test time with the demonstration data collected via the baseline collection methods and \system.  In order to ensure fairness and consistency in evaluating the various methods, we conducted tests on the trained models using ten different sets of distractors. Additionally, we repeated the tests three times with different table top configurations to obtain the average performance. Through the analysis, we draw two main insights.

\textbf{\system enables collection of demonstrations using personalized objects to train manipulation policies.} In general, the demonstration data collected either through simulation or using the PerAct VR interface (without the inclusion of personalized objects) tends to underperform due to the unavailability of these personalized objects, which are presented during testing. These findings underscore the significance of our approach, which facilitates access to collecting demonstrations with such personalized objects. Moreover, they indicate that behavior cloning (BC) models, such as PerAct, require exposure to analogous objects during demonstration to successfully execute tasks involving these objects during testing. 

\textbf{Data collected using \system yields success rates that are comparable to that collected using the real-robot system.} Referencing Table \ref{tab:press_push_pick_table}, it is evident that even with the integration of these personalized objects during the demonstration data collection phase, our methods deliver comparable results to data amassed via PerAct's VR interface using a real robot. Remarkably, our system even surpasses the performance of the PerAct VR Interface (which incorporates personalized objects) in tasks such as pushing the LEGO train and picking up the paper bag. While for the remaining personalized objects, our approach maintains a $\leq 14.3 \% $ gap across the three foundational skills.


% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=\linewidth]{images/diagnostic (2).png}
%     \caption{Your Figure}
%     \label{fig:fig5}
% \end{figure}




% \begin{wrapfigure}{r}{0.4\textwidth}
% %   \vspace{-1.3em}
% %   \vspace{-2.3em}
% %   \vspace{-4.3em}
  
%   \begin{center}
%     \vspace{-0.8cm}
%     % \hspace{2.5cm}
%     \includegraphics[width=0.42\textwidth]{diagnostic.png}

% %   \vspace{-1.2em}
%   \vspace{-0.05cm}
%   \caption{\textbf{Ablation Experiments.} Success rate of \model~after ablating key components.}
%   \label{fig:your_figure}
%   \end{center}
%   \vspace{-1em}
% %   \vspace{-1.7em}
% %   \vspace{-0.5em}
% \end{wrapfigure}
% \vspace{-0.4em}
% \hspace{-2.5cm}
% \vspace{-0.05cm}
% \textbf{Ablations.} \tabref{table:rlbench} reports \model~w/o Lang, an agent without any language conditioning. Without a language goal, the agent does not know the underlying task and performs at chance. We also report additional ablation results on the \texttt{open drawer} task in \figref{fig:ablations}. To summarize these results: (1) the skip connection helps train the agent slightly faster, (2) the Perceiver Transformer is crucial for achieving good performance with the global receptive field, and (3) extracting good keyframes actions is essential for supervised training as randomly chosen or fixed-interval keyframes lead to zero-performance.
\begin{wraptable}{r}{0.52\textwidth}
  %\begin{table}[h]
%   \hspace*{-1em}
%   \vspace{-0.5cm}
  \vspace{-1.3em}
  \setlength\tabcolsep{2.3pt}
  \centering
  \scriptsize
\begin{tabular}{lcc} 
\toprule
Task          & 2D data (Image-BC)~ & 3D data (PerAct)  \\ 
\midrule
Press the buzzer from the side & 0.00\%         & 40.00\%    \\
Pick up the queen piece    & 6.67\%         & 33.34\%           \\
Press the computer mouse    & 6.67\%        & 40.00\%           \\
\bottomrule
\end{tabular}
%   \vspace{-0.5em}
    \caption{\textbf{Training with Different Data Modalities.} AR2-D2 is capable of offering diverse data modalities to facilitate training BC models, such as Image-BC for 2D data and PerAct for 3D data. We assess these disparate data modalities, gathered via AR2-D2, across three distinct tasks using Image-BC for 2D data and PerAct for 3D data, conducted without any form of fine-tuning} % task, success \% vs. $\#$ of demonstrations. 
  \vspace{-2em}
  \label{table:table2}
\end{wraptable}

\subsection{Ablative Studies}
\textbf{Analysis on Fine-tuning.} To find the most effective iteration and demonstration combination for real-world fine-tuning, we conduct an analysis by varying the number of fine-tuning demonstrations, $D = \{1, 3, 5, 10, 15\}$, and iterations, $I = \{0, 1000, 2000, 3000, 4000, 5000\}$, during model fine-tuning and measuring the corresponding success rate. Specifically, for pre-training, we use five demonstrations totalling 30,000 iterations of the ``mouse" pressing task, collected using   AR2-D2. Following pre-training, we fine-tune with real-world demonstrations. Each resulting model is tested on five real-world scenes which has varying target object poses and distraction objects. We illustrate the experimental results in Table \ref{fig:ablations}, which indicate that utilizing 5 demonstrations of real-world foundational skills and training for 3,000 iterations (equivalent to 10 minutes of training) yields the most effective outcome.

% In Figure \ref{fig:diagnostic_analysis}, we investigate the relationship between the number of real-world fine-tuning demonstrations and the number of iterations for fine-tuning  towards the performances of tasks for demonstrations collected via   AR2-D2.  We conducted an analysis by gathering five demonstrations of pressing the "mouse" using   AR2-D2 and pre-training it for 30,000 iterations. Subsequently, we fine-tuned the pre-trained model by varying the number of real-world demonstrations and training iterations in five different instances of a test scene, with the positions of the target object and distractor also varied. This allowed us to calculate the average success rate for each combination of demonstrations and iterations. The results of this diagnostic study indicate that utilizing 5 demonstrations of real-world foundational skills and training for 3,000 iterations (equivalent to 10 minutes of training) yielded the most effective outcomes.


\textbf{Training with Different Data Modalities.} \system facilitates collection of both 2D image data and 3D depth data, which enables training of both image-based behaviour cloning (Image-BC) and 3D voxelized methods like PerAct \cite{shridhar2022perceiver}. In Table \ref{table:table2}, we show the performance of Image-BC and PerAct, trained using 2D image and 3D voxel input, respectively. We demonstrate that in a zero-shot setting, where the training data is collected in AR using \system and inference is run directly on real-world sensor input without fine-tuning, \system enables successful task execution for pushing, picking, and pressing style tasks. Specifically, we find that while models trained using 2D and 3D are capable of performing pushing, picking, and pressing style tasks, incorporating 3D information enhances the success rate by a large margin, as shown in Figure Table \ref{table:table2}. 

% of  data  enable some level of successful task execution. However, when 3D information is incorporated, the success rate significantly outperforms the Image-BC which only incorporates 2D information. 


% image data only, the Image-BC model achieves Specifically,   leverages real-world data is directly run on the for the task of \emph{pressing the cross button from the side}, in a zero-shot setting (without finetuning), we can achieve...

% To investigate the validity of different modalities collected using \system, we leverage the data to train an image-based behaviour cloning agent and Perceiver Actor. 


% To demonstrate the  To investigate the  

% Figure XXX presents an experiment investigating the influence of various input data modalities on the performance of behavior cloning agents trained to execute the task of \emph{pressing the cross button from the side}, which necessitates rotating the robot's end-effector. The experiment involves two models, namely PerAct \cite{shridhar2022perceiver} and Image-BC, and three sets of input modalities. 


% 1) train a image-BC agent, which is an image-to-action
% agent similar to BC-Z [12]. The image-BC model using RGB frames generated through our cross-reality perception pipeline. 2) A 3D voxel inputs from the    AR2-D2 onboard device sensor, which are combined with real-world action demonstrations and fine-tuned on the PerAct model. 3) A 3D voxel inputs from the    AR2-D2 onboard device sensor without any fine-tuning. All of these three models are trained for 30,000 iterations on 5 demonstrations collected via    AR2-D2.

% Figure XXX presents an experiment investigating the influence of various input data modalities on the performance of behavior cloning agents trained to execute the task of \emph{pressing the cross button from the side}, which necessitates rotating the robot's end-effector. The experiment involves two models, namely PerAct and Image-BC, and three sets of input modalities. 1) training the Image-BC model using RGB frames generated through our cross-reality perception pipeline. 2) A 3D voxel inputs from the    AR2-D2 onboard device sensor, which are combined with real-world action demonstrations and fine-tuned on the PerAct model. 3) A 3D voxel inputs from the    AR2-D2 onboard device sensor without any fine-tuning. All of these three models are trained for 30,000 iterations on 5 demonstrations collected via    AR2-D2.



==> old/introduction_old.tex <==

\section{Introduction}

% MAIN RESULTS:
% 1: system
% 2: robot can learn to manipulate objects that have never been interacted with a real robot. 
% 3: can now train a robot to interact with a personalized objects that is not obtainable en masse
% 4: manipulation results are as successful as those collected using real demonostrations with a real robot
% 5: users find it easy to use, as fast as kinesthetic data collection, human learning curve is faster, no training
% minor ablations: optimal number of demonstrations for finetuning, rbg-only variants, learning from simulation.


% Overall layout of the introduction.
% Para 1: robot data collection is really vital and powers a lot of machine learning, especially in robotics
Manually curated datasets are often the inglorious heroes of many large-scale machine learning projects~\cite{radford2021learning,ramesh2022hierarchical, duan2022survey}; this is especially true in robotics, where human-generated datasets of robot demonstrations are indispensable~\cite{dasari2019robonet,ebert2021bridge} especially with recent success in robot learning via imitation learning \cite{shridhar2022perceiver,wang2023mimicplay,ahn2022can,} of these demonstration data.
%Since pure reinforcement learning requires an immense amount of simulations for robot agents to uncover useful behavior, behavior cloning from human demonstrations has become the de-facto training mechanism to initialize agents~\cite{duan2017one}.
For example, one recent effort collected $\sim130k$ robot demonstrations, collected with a fleet of $13$ robots over the course of $17$ months~\cite{brohan2022rt}.
As a result, researchers have spent considerable effort developing various mechanisms for demonstration collection. 
One popular option is kinesthetic-teaching, where a person guides a robot through a desired trajectory~\cite{argall2009survey}. Although intuitive, this mechanism can be tedious and slow~\cite{osentoski2010crowdsourcing}. Alternatively, teleoperation with various controllers have become popular: using a keyboard and mouse~\cite{kent2017comparison,leeper2012strategies}, a video game controller~\cite{laskey2017comparing}, a 3D-mouse~\cite{dragan2012online,shridhar2022perceiver}, special purpose master-slave interfaces~\cite{akgun2012novel,liang2017using}, and even virtual reality (VR) controllers~\cite{whitney2019comparing,zhang2018deep,lipton2017baxter}.


% Para 2: robot data collection is really challenging because people need to be trained to use methods to operate real robots; on top of that, data collection is limited by how bulky robots are: they are stuck in `warehouses'. To make matters worse, robots are expensive and demonstration collection is limited by the number of available robots.
Despite all these demonstration collection efforts, there are three key challenges limiting robot data collection. First, people need to be trained to produce useful demonstrations: kinesthetic methods are labor-intensive while teleoperation methods require learning specialized controllers. 
Second, the ability to parallelize data collection is limited by how many—often expensive—robots are available. Third, robots are usually bulky and locked within a laboratory, reducing their exposure to a handful of nearby objects.


% Para 3: To make robot demonstrations collection effortless, we introduce \system. Describe what it is.

We introduce \system: a system for collecting robot demonstrations that (1) without the need to train people, (2) without any real robots during data collection, and therefore, (3) enabling manipulation of diverse objects.
\system\ is an iOS app that enables users can use to record a video of themselves manipulating any object. Once the video is captured, \system\ uses the iOS depth sensor to place an AR robot in the scene and uses a motion planner to produce a trajectory where it appears as if the AR robot manipulates the object (Figure~\ref{fig:teaser}).
Manipulating objects and recording a video is so intuitive that users do not need any training to use \system. Our system completely removes the need for a real robot during demonstration collection, allowing data collection to potentially parallelize without being limited by expensive real robots. Finally, since videos can be captured anywhere, \system\ re-situates demonstration collection out of the laboratory; users can take videos anywhere, making it easy to collect demonstrations manipulating diverse objects.




% Para 4: Lay out the experiments that were run and what the main findings were.
Our experiments show that \system's AR demonstrations can effectively train a real robot to manipulate real-world objects.
We collect and use as few as five effortlessly collected demonstrations to train a behavior cloning agent~\cite{shridhar2022perceiver}.
This trained agent needs to be finetuned for 3,000 iterations (which is equivalent to less than 10 minutes of training) on a dummy real-world task to overcome the sim-to-real gap; Once finetuned, a real robot is capable of manipulating real objects even though that object was only encountered by the AR robot.
Across three manipulation tasks (\emph{press}, \emph{pick-up} and \emph{push}) on 9 personalized objects. These personalized objects are uniquely shaped, sized, or configured items designed to meet the specific needs or functionalities of individual users within their personalized environment. This AR-trained agent performs comparable to agents trained with real-world tele-operated demonstrations (specifically the PerAct demonstration collection~\cite{shridhar2022perceiver}).

% Para 5: Lay out the user study and the main results there.
We also evaluate \system's usability by conducting a within-subjects user study (N=10). For the user study, participants are asked to provide demonstrations for two standard manipulation task: \emph{pick-up} and \emph{stacking}. Aside from \system, users also collect demonstrations using four other collection methods, including keyboard and mouse \cite{mittal2023orbit}, VR controller \cite{Shridhar2022PerceiverActorAM}, 3D-mouse \cite{mittal2023orbit}, and kinesthetic-teaching \cite{ajaykumar2021designing}.
Our results indicate that users find \system\ intuitive to use and require no training. Users even produce demonstrations as fast as kinesthetic teaching, and much faster than all other methods.
\system opens up the possibility of democratizing robot training: anyone with an iphone, which is estimated to be 1.36 billion\footnote{Source: \url{https://www.bankmycell.com/blog/number-of-iphone-users}} people in the world, will have the ability to produce personalized manipulation data that could be used to train a real robot to manipulate their personal household objects.

% \rk{Only badly written papers have a contribution list at the end. If you write a good introduction, the contributions are obvious and you don't have to list them. I am strongly against contribution lists at the end of introduction sections.}
% In summary, our contributions are as follows:
% \begin{itemize}
%     \item A \textbf{novel augmented reality perception system} designed specifically for the collection of trainable robot demonstrations in personalized environments, specifically focusing on customized objects.
%     \item A comprehensive user-study to assess the \textbf{usability} of our proposed system in comparison to conventional demonstration approaches.
%     \item  \textbf{Empirical results} from real-world tasks that demonstrates the comparable quality of the demonstrations collected through our system when compared to demonstrations obtained from real-world robot interactions.
% \end{itemize}


\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{images/figure1_2.png}
    \caption{\textbf{\system\ } collects robot demonstrations without needing a real robot. \textbf{(Left)} Using \system, the user captures a video manipulating an object with their arm. \system projects an operational URDF of an AR Franka Panda robot arm into a physical environment. It uses a hand-pose tracking algorithm to move the AR robot's end effector to align with and mirror the 6D pose of the human hand. \textbf{(Middle)} With this video demonstration, we train a perceiver-actor agent and \textbf{(Right)} deploy the agent on a real-world robot to demonstrate its ability to learn from AR demonstrations.}
    % \rk{Changes still left: (1) I want the three parts to be a bit symmetric in width. Can we change the left side to also have 4 images that take up the same amount of horizontal space? (2) Can make the images on the left smaller all the font in the figures a bit bigger?}\textcolor{red}{fixed}}
    \label{fig:teaser}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{images/figure2_1.png}
    \caption{\textbf{\system\ collection process}. \textbf{(Left)} Once the user records themselves manipulating an object, \system\ extracts the following information: 6D hand pose, hand state, RGB frames and depth estimations. We replace the hand with an AR robot, aligning its motions to align its end effector with the hand's. \textbf{(Right)} We create a 3D voxelized representation over time from the extracted information. 
    This 3D representation is used to train a \model~\cite{shridhar2022perceiver} agent. 
    We also use the processed video with the AR robot to train an image-conditioned behavior cloning agent \cite{shridhar2022perceiver}.
    % \rk{Looks better. I think we can improve it a bit further: (1) Align all the images so that all the top row are the same height and width and are aligned at the top. Notice how right now the right side has images that are taller and narrower? That doesn't look good. (2) Can we make the images slightly smaller overall and the text font slightly bigger?}\textcolor{red}{fixed the spacing}
    }
    \label{fig:fig2}
\end{figure}


==> old/introduction_v1.tex <==

\section{Introduction}
\label{sec:intro}


% In recent years, the field of robotics has experienced significant growth and advancements \cite{duan2022survey,shridhar2022perceiver,agarwal2022legged}. In particular, several algorithms have emerged in robotic manipulation to enable robots to learn skills through demonstrations. However, a key challenge that exists is collecting data of sufficient scale to train algorithms that can perform robustly in diverse environments. Existing methods have 


% is providing examples to teach necessary skills.
% Key points:
% - How to train robots: rl & il are two mainstream approaches
% - Robotics needs data
% - Popular data collection methods

% 



In recent years, the field of robotics has experienced significant growth and advancements \cite{duan2022survey,shridhar2022perceiver,agarwal2022legged}. These advancements have led to the development of complex and sophisticated robot learning agents that utilize transformers tailored for robot learning and are grounded on language \cite{wei2022chain,ramesh2022hierarchical,alayrac2022flamingo} and large-scale demonstrations\cite{brohan2022rt}. However, training these robots to perform specific tasks solely through reinforcement learning can be a challenging and time-consuming process. One potential solution to address this challenge is the application of imitation learning\cite{duan2017one}, particularly through supervised training utilizing human tele-operated demonstrations or expert policy trajectories generated by motion planners in simulation. Despite the promise of these new transformer models that focus on training imitation learning agents for general-purpose tasks, there still exists a bottleneck in the supervised approaches, necessitating the collection of large-scale and diverse demonstrations across various environments. The collection of robot demonstrations is a time-consuming and labor-intensive task. Additionally, obtaining high-quality training data for training behavior cloning agents requires users to possess a certain level of visualization of the robot embodiment and perform highly specific actions to gather this trainable data. These requirements cannot be fulfilled solely through ego-centric video datasets such as Ego4D. The majority of high-quality robot demonstration data must be collected by users teleoperating real robots, which poses significant challenges for scalability across a diverse range of environments.

In order to facilitate the scalability of imitation learning in robot manipulation across various environments, there is a pressing need for an intuitive and scalable approach to collect large-scale robot demonstrations in individuals' personalized homes, specifically involving customized objects. Ideally, this approach should eliminate the necessity of utilizing a physical robot. To address this need, we propose the implementation of JARVIS, an augmented reality mobile application. JARVIS allows users to project a fully functional Franka Panda Robot Arm with 6D end-effector control into their personalized environment. This projection is achieved through hand tracking, enabling users to collect robot manipulation demonstrations with customized objects. Some iPhone or iPad devices are equipped with built-in depth sensors, which enables us to capture precise depth information. This depth information is utilized to generate 3D voxel inputs, along with the robot's keyframe 6-DoF pose. These inputs are crucial for training language-conditioned behavior cloning (BC) agents, using state-of-the-art robot learning transformer models such as Perceiver-Actor (PerAct). Once the BC agents are trained, their policies can be deployed into the real world, allowing them to perform manipulation tasks on the customized objects in diverse scenes. This integration of augmented reality, depth sensing, and transformer-based models empowers JARVIS to collect demonstrations and train effective robot manipulation policies in the real-world. 

To assess the usability of the JARVIS system for data collection purposes, we conducted an extensive user study. The study aimed to benchmark various methods of collecting robot manipulation demonstrations, including both real-world robot interactions and simulations. Additionally, we sought to investigate the quality of the demonstration data obtained through JARVIS, specifically for training behavior cloning (BC) agents. To accomplish this, we pretrained demonstrations collected from real-world interactions, simulations, and JARVIS. We then fine-tuned these demonstrations using three sets of foundational tasks (\emph{press}, \emph{pick} and \emph{push}) with a collection of customized objects that were not previously encountered during the fine-tuning process. Our results demonstrate that JARVIS performs comparably to robot demonstrations collected using the PerAct robot data collection interface.

In summary, our contributions are as follows:
\begin{itemize}
    \item A \textbf{novel augmented reality perception system} designed specifically for the collection of trainable robot demonstrations in personalized environments, specifically focusing on customized objects.
    \item A comprehensive user-study to assess the \textbf{usability} of our proposed system in comparison to conventional demonstration approaches.
    \item  \textbf{Empirical results} from real-world tasks that demonstrates the comparable quality of the demonstrations collected through our system when compared to demonstrations obtained from real-world robot interactions.
\end{itemize}



% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=\textwidth]{figure 2.png}
%     \caption{Training JARVIS pipeline.}
%     \label{fig:full-image}
% \end{figure}
% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=\textwidth]{images/figure2.png}
%     \caption{Different approaches of collecting robot demonstration via JARVIS and the different input modalities. (Top) Hand pose control. (Middle) Programmable replay. (Bottom) AR Kinesthetic. }
%     \label{fig:control}
% \end{figure}


\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{images/Untitled.jpg}
    \caption{Training JARVIS pipeline.}
    \label{fig:full-image}
\end{figure}


\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{images/figure1.jpg}
    \caption{Training JARVIS pipeline.}
    \label{fig:full-image}
\end{figure}


==> old/introduction_v2.tex <==

\section{Introduction}

% MAIN RESULTS:
% 1: system
% 2: robot can learn to manipulate objects that have never been interacted with a real robot. 
% 3: can now train a robot to interact with a personalized objects that is not obtainable en masse
% 4: manipulation results are as successful as those collected using real demonostrations with a real robot
% 5: users find it easy to use, as fast as kinesthetic data collection, human learning curve is faster, no training
% minor ablations: optimal number of demonstrations for finetuning, rbg-only variants, learning from simulation.


% Overall layout of the introduction.
% Para 1: robot data collection is really vital and powers a lot of machine learning, especially in robotics
Manually curated datasets are often the inglorious heroes of many large-scale machine learning projects~\cite{radford2021learning,ramesh2022hierarchical}; this is especially true in robotics, where human-generated datasets of robot demonstrations are indispensable~\cite{dasari2019robonet,ebert2021bridge}.
%Since pure reinforcement learning requires an immense amount of simulations for robot agents to uncover useful behavior, behavior cloning from human demonstrations has become the de-facto training mechanism to initialize agents~\cite{duan2017one}.
For example, one recent effort collected $\sim130k$ robot demonstrations, collected with a fleet of $13$ robots over the course of $17$ months~\cite{brohan2022rt}.
As a result, researchers have spent considerable effort developing various mechanisms for demonstration collection. 
One popular option is kinesthetic-teaching, where a person guides a robot through a desired trajectory~\cite{argall2009survey}. Although intuitive, this mechanism can be tedious and slow~\cite{osentoski2010crowdsourcing}. Alternatively, teleoperation with various controllers have become popular: using a keyboard and mouse~\cite{kent2017comparison,leeper2012strategies}, a video game controller~\cite{laskey2017comparing}, a 3D-mouse~\cite{dragan2012online,shridhar2022perceiver}, special purpose master-slave interfaces~\cite{akgun2012novel,liang2017using}, and even virtual reality~\cite{whitney2019comparing,zhang2018deep,lipton2017baxter}.


% Para 2: robot data collection is really challenging because people need to be trained to use methods to operate real robots; on top of that, data collection is limited by how bulky robots are: they are stuck in `warehouses'. To make matters worse, robots are expensive and demonstration collection is limited by the number of available robots.
Despite all these demonstration collection efforts, there are three key challenges limiting robot data collection. First, people need to be trained to produce useful demonstrations: kinesthetic methods are labor-intensive while teleoperation methods require learning specialized controllers. 
Second, the ability to parallelize data collection is limited by how many—often expensive—robots are available. Third, robots are usually bulky and locked within a laboratory, reducing their exposure to a handful of nearby objects.


% Para 3: To make robot demonstrations collection effortless, we introduce \system. Describe what it is.

We introduce \system: a system for collecting robot demonstrations that (1) without the need to train people, (2) without any real robots, and therefore, (3) enabling manipulation of diverse objects.
\system\ is an iOS app that enables users can use to record a video of themselves manipulating any object. Once the video is captured, \system\ uses the iOS depth sensor to place an AR robot in the scene and uses inverse kinetics to produce a trajectory where it appears as if the AR robot manipulates the object (Figure~\ref{fig:teaser}).
Manipulating objects and recording a video is so intuitive that users do not need any training to use \system. Our system completely removes the need for a real robot, allowing data collection to potentially parallelize without being limited by expensive real robots. Finally, since videos can be captured anywhere, \system\ re-situates demonstration collection out of the laboratory; users can take videos anywhere, making it easy to collect demonstrations manipulating diverse objects.




% Para 4: Lay out the experiments that were run and what the main findings were.



% Para 5: Lay out the user study and the main results there. End by saying that this opens up the possibility of demonstratizing robot training: where anyone with an iphone, which is X percentage of people in the world, will have the capacity to produce training data to personalize a robot to manipulate specific objects of their interest.


To assess the usability of the JARVIS system for data collection purposes, we conducted an extensive user study. The study aimed to benchmark various methods of collecting robot manipulation demonstrations, including both real-world robot interactions and simulations. Additionally, we sought to investigate the quality of the demonstration data obtained through JARVIS, specifically for training behavior cloning (BC) agents. To accomplish this, we pretrained demonstrations collected from real-world interactions, simulations, and JARVIS. We then fine-tuned these demonstrations using three sets of foundational tasks (\emph{press}, \emph{pick} and \emph{push}) with a collection of customized objects that were not previously encountered during the fine-tuning process. Our results demonstrate that JARVIS performs comparably to robot demonstrations collected using the PerAct robot data collection interface.

In summary, our contributions are as follows:
\begin{itemize}
    \item A \textbf{novel augmented reality perception system} designed specifically for the collection of trainable robot demonstrations in personalized environments, specifically focusing on customized objects.
    \item A comprehensive user-study to assess the \textbf{usability} of our proposed system in comparison to conventional demonstration approaches.
    \item  \textbf{Empirical results} from real-world tasks that demonstrates the comparable quality of the demonstrations collected through our system when compared to demonstrations obtained from real-world robot interactions.
\end{itemize}


\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{images/figure1.png}
    \caption{Training JARVIS pipeline.}
    \label{fig:teaser}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{images/figure2.png}
    \caption{Training JARVIS pipeline.}
    \label{fig:full-image}
\end{figure}

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=\textwidth]{images/figure1.jpg}
%     \caption{Training JARVIS pipeline.}
%     \label{fig:full-image}
% \end{figure}


==> old/introduction_v3.tex <==

\section{Introduction}

% MAIN RESULTS:
% 1: system
% 2: robot can learn to manipulate objects that have never been interacted with a real robot. 
% 3: can now train a robot to interact with a personalized objects that is not obtainable en masse
% 4: manipulation results are as successful as those collected using real demonostrations with a real robot
% 5: users find it easy to use, as fast as kinesthetic data collection, human learning curve is faster, no training
% minor ablations: optimal number of demonstrations for finetuning, rbg-only variants, learning from simulation.


% Overall layout of the introduction.
% Para 1: robot data collection is really vital and powers a lot of machine learning, especially in robotics
Manually curated datasets are often the inglorious heroes of many large-scale machine learning projects~\cite{radford2021learning,ramesh2022hierarchical}; this is especially true in robotics, where human-generated datasets of robot demonstrations are indispensable~\cite{dasari2019robonet,ebert2021bridge}.
%Since pure reinforcement learning requires an immense amount of simulations for robot agents to uncover useful behavior, behavior cloning from human demonstrations has become the de-facto training mechanism to initialize agents~\cite{duan2017one}.
For example, one recent effort collected $\sim130k$ robot demonstrations, collected with a fleet of $13$ robots over the course of $17$ months~\cite{brohan2022rt}.
As a result, researchers have spent considerable effort developing various mechanisms for demonstration collection. 
One popular option is kinesthetic-teaching, where a person guides a robot through a desired trajectory~\cite{argall2009survey}. Although intuitive, this mechanism can be tedious and slow~\cite{osentoski2010crowdsourcing}. Alternatively, teleoperation with various controllers have become popular: using a keyboard and mouse~\cite{kent2017comparison,leeper2012strategies}, a video game controller~\cite{laskey2017comparing}, a 3D-mouse~\cite{dragan2012online,shridhar2022perceiver}, special purpose master-slave interfaces~\cite{akgun2012novel,liang2017using}, and even virtual reality (VR) controller~\cite{whitney2019comparing,zhang2018deep,lipton2017baxter}.


% Para 2: robot data collection is really challenging because people need to be trained to use methods to operate real robots; on top of that, data collection is limited by how bulky robots are: they are stuck in `warehouses'. To make matters worse, robots are expensive and demonstration collection is limited by the number of available robots.
Despite all these demonstration collection efforts, there are three key challenges limiting robot data collection. First, people need to be trained to produce useful demonstrations: kinesthetic methods are labor-intensive while teleoperation methods require learning specialized controllers. 
Second, the ability to parallelize data collection is limited by how many—often expensive—robots are available. Third, robots are usually bulky and locked within a laboratory, reducing their exposure to a handful of nearby objects.


% Para 3: To make robot demonstrations collection effortless, we introduce \system. Describe what it is.

We introduce \system: a system for collecting robot demonstrations that (1) without the need to train people, (2) without any real robots during data collection, and therefore, (3) enabling manipulation of diverse objects.
\system\ is an iOS app that enables users can use to record a video of themselves manipulating any object. Once the video is captured, \system\ uses the iOS depth sensor to place an AR robot in the scene and uses a motion planner to produce a trajectory where it appears as if the AR robot manipulates the object (Figure~\ref{fig:teaser}).
Manipulating objects and recording a video is so intuitive that users do not need any training to use \system. Our system completely removes the need for a real robot during demonstration collection, allowing data collection to potentially parallelize without being limited by expensive real robots. Finally, since videos can be captured anywhere, \system\ re-situates demonstration collection out of the laboratory; users can take videos anywhere, making it easy to collect demonstrations manipulating diverse objects.




% Para 4: Lay out the experiments that were run and what the main findings were.
Our experiments show that \system's AR demonstrations can effectively train a real robot to manipulate real-world objects.
We collect and use as few as five effortlessly collected demonstrations to train a behavior cloning agent~\cite{shridhar2022perceiver}.
This trained agent needs to be finetuned for 3,000 iterations (which is equivalent to less than 10 minutes of training) on a dummy real-world task to overcome the sim-to-real gap; Once finetuned, a real robot is capable of manipulating real objects even though that object was only encountered by the AR robot.
Across three manipulation tasks (\emph{press}, \emph{pick} and \emph{push}) on 9 personalized objects, this AR-trained agent performs comparable to agents trained with real-world tele-operated demonstrations (specifically the PerAct demonstration collection~\cite{shridhar2022perceiver}).

% Para 5: Lay out the user study and the main results there.
We also evaluate \system's usability by conducting a within-subjects user study (N=10). Participants are asked to provide demonstrations to manipulate a set of 9 personalized objects across the three manipulation tasks. Aside from \system, users also collect demonstrations using four other collection methods, including keyboard and mouse \cite{mittal2023orbit}, VR controller \cite{Shridhar2022PerceiverActorAM}, 3D-mouse \cite{mittal2023orbit}, and kinesthetic-teaching \cite{ajaykumar2021designing}.
Our results indicate that users find \system\ intuitive to use and require no training. Users even produce demonstrations as fast as kinesthetic teaching, and much faster than all other methods.
\system opens up the possibility of democratizing robot training: anyone with an iphone, which is estimated to be 1.36 billion\footnote{Source: \url{https://www.bankmycell.com/blog/number-of-iphone-users}} people in the world, will have the ability to produce personalized manipulation data that could be used to train a real robot to manipulate their personal household objects.

% \rk{Only badly written papers have a contribution list at the end. If you write a good introduction, the contributions are obvious and you don't have to list them. I am strongly against contribution lists at the end of introduction sections.}
% In summary, our contributions are as follows:
% \begin{itemize}
%     \item A \textbf{novel augmented reality perception system} designed specifically for the collection of trainable robot demonstrations in personalized environments, specifically focusing on customized objects.
%     \item A comprehensive user-study to assess the \textbf{usability} of our proposed system in comparison to conventional demonstration approaches.
%     \item  \textbf{Empirical results} from real-world tasks that demonstrates the comparable quality of the demonstrations collected through our system when compared to demonstrations obtained from real-world robot interactions.
% \end{itemize}


\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{images/figure1.png}
    \caption{\textbf{\system\ } collects robot demonstrations without needing a real robot. \textbf{(Left)} Using \system, the user captures a video manipulating an object with their arm. \system projects an operational URDF of an AR Franka Panda robot arm into a physical environment. It uses a hand-pose tracking algorithm to move the AR robot's end effector to align with and mirror the 6D pose of the human hand. \textbf{(Middle)} With this video demonstration, we train a perceiver-actor agent and \textbf{(Right)} deploy the agent on a real-world robot to demonstrate its ability to learn from AR demonstrations. 
    \rk{I would like to improve this image. Here are the list of changes I recommend: (1) I want the three parts to be a bit symmetric. Can we change the left side to also have 4 images of the hand manipulating an object? Maybe add the AR photo only in the last of the 4 frames? (2) Can we unbold everything? (3) Can we use a better font? Lato is a good option. But I am open to other sans-serifs. (4) Can we make ALL the arrows grey and a little bit narrower to de-emphasize them? (5) All the 4 robot images can have their sides cropped to take up less width.}}
    \label{fig:teaser}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{images/figure2.png}
    \caption{\textbf{\system\ collection process}. \textbf{(Left)} Once the user records themselves manipulating an object, \system\ extracts the following information: 6D hand pose, hand state, RGB frames and depth estimations. We replace the hand with an AR robot, aligning its motions to align its end effector with the hand's. \textbf{(Right)} We create a 3D voxelized representation over time from the extracted information. 
    This 3D representation is used to train a \model~\cite{shridhar2022perceiver} agent. 
    We also use the processed video with the AR robot to train a image-conditioned behavior cloning agent \cite{shridhar2022perceiver}.
    \rk{cite here if you cite \model\ in the previous sentence.}
    \rk{Figure changes: (1) remove the dotted lines. Always use white space to denote gestalt grouping and never use boundaries. (2) Change the first column header to be ``Data extracted from phone application'', change the second column header to be ``Generated training data''. (3) same as last figure: unbold everything and use a better font. (4) Everywhere in the paper, make sure that all headers only have the first word capitalized and no subsequent word. (5) Make the left column and right column take up the same amount of horizontal space. (6) Drop all the citation numbers. (7) Change ``Extracted Frames'' to ``Voxelized input with highlighted manipulation keypoint''.}
    }
    \label{fig:fig2}
\end{figure}


==> old/method_v1.tex <==
\section{The \system system}

We introduce AR2-D2, a system for collecting robot demonstrations without requiring a physical robot. In this section, we describe \system's features, its supported data collection procedure, its implementation details. 
% We also conduct an user study contrasting our system against others.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/figure3.jpg}
    \caption{\textbf{Language-Guided Manipulation Tasks using AR2-D2 Demonstration Collection}: We employ AR2-D2 as a tool for gathering a diverse array of manipulations encompassing three fundamental actions, involving a wide variety of customized objects. These manipulations range from performing precise actions such as pressing a computer mouse or a Minecraft torch button at specific locations, to pushing small LEGO train toys towards table-sized drawers, and even encompassing the ability to pick up objects varying from chess pieces to takeaway bags. By leveraging a limited number of real-world action demonstrations conducted with random dummy objects and fine-tuning for 3,000 iterations which is equivalent to 10 minutes of training, we have achieved the capacity to apply the PerAct framework in manipulating all these personalized objects with broad generalization.}
    \label{fig:diagnostic_analysis}
\end{figure}

\subsection{\system\ system features}
\system\ contributes the following features:

\textbf{No need for a physical robot.} In traditional robotics research, obtaining demonstrations often involves operating a physical robot~\cite{finn2017one,billard2008robot,zhang2018deep,song2020grasping}. \system\ presents a new paradigm for collecting demonstrations; it forgoes access to a real robot, enabling users to collect high-quality demonstration data from anywhere with only their mobile devices. 

\textbf{Real-time control of AR robots in the real-world.} \system\ leverages LiDAR sensors, which today are ubiquitous in iPhones and other smartphones to estimate the 3D layout in front of the camera to project an AR robot. LiDAR helps the AR robot obey physical and visual realism. Users can control the AR robot in one of three supported interactions: by pointing at 3D points that the robot's end-effector should move to, by using the iPhone's GUI control, or through AR kinesthetic control. The projected robot's motions are tightly coupled with the real-world environment, and receives feedback upon collisions with real-world objects.


\textbf{Real-time visualization of task feasibility.} \system\ simplifies the demonstration collection by asking users to specify key-points that the robot end-effector should move to in order to complete a task. Once each key-point is specified, \system\ visualizes the AR robot's motion, moving its end-effector from its current position to the new specified key-point. This real-time feedback enables users to assess the feasibility and accuracy of the specified key-point and revise their selections if necessary.

\subsection{Design and implementation}

\system's design and implementation consists of two primary components (Figure \ref{fig:fig2}).
The first component is a phone application that projects AR robots into the real-world, allowing users to interact with physical objects and the AR robot. The second component convert collected videos into a format that can be used to train different behavior cloning agents, which can later be deployed on real robots.

\textbf{The phone application.} 
We designed \system\ as an iOS application, which can be run on an iPhone or iPad. Since modern mobile devices and tablets come equipped with in-built LiDAR, we can effectively place AR robots into the real world. 
The phone application is developed atop the Unity Engine and the AR Foundation kit. The application receives camera sensor data, including camera intrinsic and extrinsic values, and depth directly from the mobile device's built-in functionality. The AR Foundation kit enables the projection of the Franka Panda robot arm's URDF into the physical space. To determine user's 2D hand pose, we utilize Apple's human pose detection algorithm. This, together with the depth map is used to reconstruct the 3D pose of the human hand. By continuously tracking the hand pose at a rate of $30$ frames per second, we can mimic the pose with the AR robot's end-effector. 



\textbf{Training data creation.} Given language instructions describing a task (e.g.~``Pick up the plastic bowl''), we hire users to generate demonstrations using the phone application. From the user-generated demonstration video, we generate training data that can be used to train and deploy on a real robot. 
To create useful training data, we convert this video into one where it looks like an AR robot manipulated the object. To do so, we segment out and eliminate the human hand using Segment-Anything~\cite{kirillov2023segment}. We fill in the gap left behind by the missing hand with a video in-painting technique known as E2FGVI~\cite{li2022towards}
Finally, we produce a video with the AR robot arm moving to the key-points identified by the user's hand. This final video processed video makes it appear as if an AR robot arm manipulated the real-world object; it can befor visual-based imitation learning~\cite{young2020visual}.
Additionally, since we have access to the scene's depth estimation, we can also generate a 3D voxelized representation of the scene and use it to train agents like Perceiver-Actor (\model)~\cite{shridhar2022perceiver}.



==> old/related_v1.tex <==
\section{Related Works}

\textbf{Data Collection Methods for Offline Learning from Demonstrations}

Imitation learning has pioneered a paradigm shift in robot training for the execution of a wide array of manipulative tasks. A primary focus in this field of study concerns offline learning from demonstrations, a process by which a policy derives knowledge from a fixed dataset of robotic demonstrations, without any supplemental interaction. This method typically employs Behavior Cloning (BC) \cite{pomerleau1988alvinn}, wherein the goal is to replicate actions from the dataset through supervised learning. The acquisition of robotic demonstrations for training BC agents generally follows two predominant strategies. The first focuses on capturing robotic demonstrations in a simulated environment, utilizing techniques such as Task and Motion Planning (TAMP) \cite{dalal2023imitating} or annotating key frames within the demonstrations \cite{james2022coarse}. The second, in contrast, emphasizes collecting robotic demonstrations in real-world settings, leveraging techniques such as teleportation, vision-based guidance, and advanced hardware capabilities \cite{finn2017one,billard2008robot,zhang2018deep}. Song et al. \cite{song2020grasping} introduced a low-cost handheld device featuring a plastic grabber tool outfitted with an RGB-D camera and a servo for controlling the binary opening and closing of the grabber fingers. Furthermore, Wang et al. \cite{wang2023mimicplay} deployed video sequences showcasing people engaging with their environments manually for the training of visual-motor policies to perform manipulative tasks. In contrast, our data collection approach centers on a hybrid model, which involves projecting a simulated robot to engage with the physical world through human hand interactions. This approach alleviates the necessity of constructing a simulator or the requirement for a physical robot. Unlike MimicPlay \cite{wang2023mimicplay}, our approach not only enables the collection of a more diverse 3D representation for training multi-task transformers like PerAct but also furnishes the data modalities necessary for training visual-motor policy
 
\textbf{Generic Task Demonstration Collection Methods for Robot Learning}
There are several conventional methods available for gathering task demonstrations to be used in generic robot learning algorithms. One popular approach involves kinesthetically controlling the robot to follow a desired trajectory, thereby showcasing the behavior required to accomplish a specific task \cite{argall2009survey}. Alternatively, teleoperation techniques \cite{goldberg1994beyond,lumelsky1993real,hokayem2006bilateral} utilizing various user interfaces such as keyboards and mouse \cite{kent2017comparison,leeper2012strategies}, video game controllers \cite{laskey2017comparing}, VR Controller \cite{perceivertransformer} 3D Space Mouse\cite{dragan2012online}, and even tracking the pose of a mobile phone to remotely control a robot arm can also be used \cite{mandlekar2018roboturk}. However, unlike our approach, all of these methods require a physical robot to be controlled at the other end, making them less accessible for collecting data in a user's personalized space.





% Imitation learning is vital for training robots, with research spanning decades. It aims to improve robot performance and adaptability by learning from expert demonstrations. Recently, significant progress has been made by integrating foundational models like CLIP\cite{radford2021learning}, BERT\cite{devlin2018bert}, and ViT\cite{yuan2021tokens}. These models have advanced imitation learning techniques. CLIP excels in visual perception and language grounding, BERT revolutionizes natural language processing for applications like instruction following and human-robot interaction, and ViT brings transformers to computer vision tasks for robotic perception and control.Another critical aspect is collecting high-quality expert demonstrations. Methods like teleportation, vision-based guidance, and crowd-sourcing aim to capture diverse demonstrations for better generalization and performance in learned policies. Song et al \cite{song2020grasping}. investigated teleportation for robotic grasping tasks, allowing remote task performance and high-quality demonstration collection. Young et al. proposed a vision-based guidance system using visual cues for real-time feedback and improved demonstration quality. Mandlekar et al \cite{mandlekar2018roboturk}. introduced Roboturk, a crowd-sourcing platform for scalable expert demonstration gathering, addressing data scarcity in imitation learning research.

% In conclusion, related works in imitation learning include developing novel algorithms based on foundational models and collecting expert demonstrations. Both aspects are crucial for the field's progress, and future research will likely explore innovative methods to enhance imitation learning efficiency and effectiveness in robotics.

% ignore these commented lines below
%   The age in which infants adopt core principles of persistence, inertia \& gravity \cite{lin2020infants} have been widely studied in a variety of event categories
%  where a \textit{surprising} scene was demonstrated with a taller object being fully contained in a shorter container, violating solidity constraints. Continuity constraints were also violated in \textbf{occluder} events \cite{baillargeon1991object, spelke1995spatiotemporal} when objects teleported behind one occluder to the back of another disconnected occluder. This event was also modified with different occluder heights in the middle segment \cite{aguiar19992}. Researchers also experimented with inertia violations in \textbf{collision} events \cite{kotovsky1994calibration, kotovsky1998development} where the outcome of the contact was impossible via linear momentum. Finally, gravity violations were also studied as \textbf{support} events \cite{baillargeon1992development, dan2000development, hespos2008young} where imbalanced objects that appeared stable were presented to infants.


==> old/related_v2.tex <==
\section{Related work}
We compare our work to existing demonstration collection methods.
 
\textbf{Demonstration collection methods.}
There are several conventional methods available for gathering robot demonstrations.
One popular approach involves kinesthetically controlling the robot to follow a desired trajectory; the generated robot trajectories showcase the behavior required to accomplish a specific task~\cite{argall2009survey}.
Teleoperation techniques~\cite{goldberg1994beyond,lumelsky1993real,hokayem2006bilateral} have also been a popular collection process, using various user interfaces including keyboard and mouse~\cite{kent2017comparison,leeper2012strategies}, a video game controller~\cite{laskey2017comparing}, 3D-mouse~\cite{dragan2012online,shridhar2022perceiver}, 3D mobile phones~\cite{mandlekar2018roboturk}, special purpose master-slave interfaces~\cite{akgun2012novel,liang2017using}, and even virtual reality controllers~\cite{whitney2019comparing,zhang2018deep,lipton2017baxter,perceivertransformer}.
However, all of these methods require a real physical robot to be controlled, bottlenecking demonstration collection by how many robots are available and limited to the laboratories that house these robots.

\textbf{Demonstrations for behavior cloning.}
Recently, robot demonstrations are primarily used as training data for imitation learning, which has pioneered a paradigm shift in robot training.
Offline behavior cloning from robot demonstrations is currently the de-facto imitation learning paradigm~\cite{pomerleau1988alvinn}. 
These demonstrations are collected either in simulation or through human control using a real robot in the real world~\cite{dalal2023imitating,james2022coarse}.
For example, Task and Motion Planning (TAMP) uses expert task planners to create large-scale simulation demonstrations~\cite{dalal2023imitating}.
Meanwhile in the real-world, users employ techniques such as teleportation or vision-based guidance are used to create demonstrations~\cite{finn2017one,billard2008robot,zhang2018deep}. 
Recent methods have also begun developing specialized hardware to streamline demonstration collection.
For example, a low-cost handheld device featuring a plastic grabber tool outfitted with an RGB-D camera and a servo can control the binary opening and closing of a grabber's fingers~\cite{song2020grasping}. 
By contrast, our real-world data collection approach requires no teleoperation hardware \cite{mandlekar2018roboturk}, no simulators\cite{james2020rlbench}, and most importantly, no real robots\cite{wu2017visual}. All we need is an iPhone camera to record users manipulating objects with their hands. 


==> old/scratch.tex <==


We introduce \system: a system for collecting robot demonstrations that (1) without the need to train people, (2) without any real robots, and therefore, (3) enabling manipulation of diverse objects.
\system\ is an iOS app that enables users can use to record a video of themselves manipulating any object. Once the video is captured, \system\ uses the iOS depth sensor to place an AR robot in the scene and uses inverse kinetics to produce a trajectory where it appears as if the AR robot manipulates the object (Figure~\ref{fig:teaser}).
Manipulating objects and recording a video is so intuitive that users do not need any training to use \system. Our system completely removes the need for a real robot, allowing data collection to potentially parallelize without being limited by expensive real robots. Finally, since videos can be captured anywhere, \system\ re-situates demonstration collection out of the laboratory; users can take videos anywhere, making it easy to collect demonstrations manipulating diverse objects.


To address this need, we propose the implementation of JARVIS, an augmented reality mobile application. JARVIS allows users to project a fully functional Franka Panda Robot Arm with 6D end-effector control into their personalized environment. This projection is achieved through hand tracking, enabling users to collect robot manipulation demonstrations with customized objects. Some iPhone or iPad devices are equipped with built-in depth sensors, which enables us to capture precise depth information. This depth information is utilized to generate 3D voxel inputs, along with the robot's keyframe 6-DoF pose. These inputs are crucial for training language-conditioned behavior cloning (BC) agents, using state-of-the-art robot learning transformer models such as Perceiver-Actor (PerAct). Once the BC agents are trained, their policies can be deployed into the real world, allowing them to perform manipulation tasks on the customized objects in diverse scenes. This integration of augmented reality, depth sensing, and transformer-based models empowers JARVIS to collect demonstrations and train effective robot manipulation policies in the real-world. 
